Explorable Super Resolution

Single image super resolution (SR) has seen major performance leaps in recent years. However, existing methods do not allow exploring the infinitely many plausible reconstructions that might have given rise to the observed low-resolution (LR) image. These different explanations to the LR image may dramatically vary in their textures and fine details, and may often encode completely different semantic information. In this paper, we introduce the task of explorable super resolution. We propose a framework comprising a graphical user interface with a neural network backend, allowing editing the SR output so as to explore the abundance of plausible HR explanations to the LR input. At the heart of our method is a novel module that can wrap any existing SR network, analytically guaranteeing that its SR outputs would precisely match the LR input, when downsampled. Besides its importance in our setting, this module is guaranteed to decrease the reconstruction error of any SR network it wraps, and can be used to cope with blur kernels that are different from the one the network was trained for. We illustrate our approach in a variety of use cases, ranging from medical imaging and forensics, to graphics.

==> ablation_study.tex <==
\section{Ablation Study Experiment Details}\label{app:ablation_study}
\yb{Should be changed - this is no longer the experiment presented:}
We performed an experiment to evaluate the effect of the two training mechanisms that encourage the effect of control input $z$, namely binding $z$ to spatial image derivatives using ${\cal L}_{\nabla^2}$ and encouraging the mapping of $z$ space to diverse plausible output images, using ${\cal L}_\mathrm{Map}$. We examined the effects of utilizing these training mechanisms in terms of the diversity, perceptual quality and reconstruction error of the yielded SR images. Results are presented in Tab.~\ref{tab:losses_ablation}, along with a comparison to the performance of ESRGAN \cite{wang2018esrgan}.

We studied the case of x4 SR and used the BSD100 dataset \cite{martin2001bsd100} (containing 100 images), and for each of our network variants produced 50 different SR images per LR input $y$, using 50 randomly sampled, spatially uniform $z$ inputs. We used the average no-reference \emph{Naturalness Image Quality Evaluator} (NIQE) score \cite{mittal2012niqe} to measure perceptual quality. As a reference, note that the average NIQE score of the original BSD100 HR images was 3.13. 

To evaluate the diversity of our networks' outputs, we used the average per-pixel standard deviation across the different $z$ inputs $\sigma_s$. Note however that since our method's outputs are consistent with their corresponding input image $y$, their diversity can only be manifested in $\hat{x}_\bot$, the component of $\hat{x}$ lying in the orthogonal subspace $\cal K_\bot$. Therefore we projected $\hat{x}$ onto $\cal K_\bot$ before calculating $\sigma$, to yield a more relevant diversity score. To put $\sigma$ values into context, note that the average spatial standard deviation of $x_\bot$ (the component of the real HR image $x$ lying in $\cal K_\bot$) is 15.18.

Finally, we used the Root Mean Square Error (RMSE) measure to quantify reconstruction error. For each output image $\hat{x}$, we measured the square differences between $\hat{x}$ and its corresponding ground truth image $x$. We then averaged over the three color channels and over the entire image, and took a square root, comprising a per image RMSE. To yield the final RMSE value, we computed the average over all 50 image versions (except for the case of ESRGAN), over each of the 100 BSD100 images.



==> boundary_effects.tex <==
\section{Boundary Effects}\label{app:boundary_effects}
Our consistency enforcing module comprises several filter convolution operations (see Fig.~\ref{fig:architechture}), each resulting in reduced output size. We follow the common practice of zero-padding filters' outputs to match their input sizes, which causes the consistency guarantee to brake, as we get closer to image boundaries, potentially resulting in undesired boundary effects.

To prevent these boundary effects from affecting the training of our editable SR network, we avoid utilizing outer image regions when calculating our loss function (Eq.~\ref{eq:total_loss}), by first cropping the $10\times\alpha$ outer pixels of our network's output, where $\alpha$ is the SR scale factor. In inference mode, we reduce boundary effects by replicating the LR image boundary pixels $10$ times, before feeding it to our network. This works better than the common zero-padding.

==> structure_tensor_loss.tex <==
\section{Utilizing Loss Term ${\cal L}_{\text{Struct}}$}\label{app:structure_tensor_loss}
As we explain in Sec.~\ref{subsec:effective_control}, we encourage control signal $z$ to affect the magnitude and direction of spatial derivatives of output image $\hat{x}$, by associating $z$ with the structure tensor of $\hat{x}$, a $2\times2$ matrix computed by
% \mbox{${\cal S}_{\hat{x}}=\begin{bmatrix}\Sigma_n s^2_x[n] & \Sigma_n s_x[n] s_y[n] \\ \Sigma_n s_x[n] s_y[n] & \Sigma_n s^2_y[n] \end{bmatrix}$}.
\mbox{${\cal S}_{\hat{x}}=\iint (\nabla \hat{x}(\xi,\eta)) (\nabla \hat{x}(\xi,\eta))^Td\xi d\eta$}.
We encode this link into our network during training by penalizing for the difference between desired, randomly sampled, image structure tensors ${\cal S}_\text{d}$, and their corresponding tensors calculated over the resulting images $\hat{x}$, ${\cal S}_\text{s}$. 

To this end, we perform the following steps for each training image:
\begin{enumerate}
    \item We uniformly sample $\lambda_{1,2}\in[0,1]$ and $\theta\in[0,2\pi]$, corresponding to magnitudes and direction of prominent image edges, respectively. These parameters induce a specific \emph{Singular Values Decomposition} (SVD) of an image structure tensor, and therefore uniquely determine it.
    \item\label{item:structure_tensor_SVD} We then compose the desired structure tensor ${\cal S}_\text{d}$: \mbox{${\cal S}_\text{d}=\begin{bmatrix}\lambda_1\cos^2{\theta}+\lambda_2\sin^2{\theta} & \lambda_1\lambda_2\sin{\theta}\cos{\theta} \\ \lambda_1\lambda_2\sin{\theta}\cos{\theta} & \lambda_1\sin^2{\theta}+\lambda_2\cos^2{\theta} \end{bmatrix}$}.
    \item We feed our network with image $y$, along with the three unique values in ${\cal S}_\text{d}$ as our control signal $z$ (uniform value per channel), after normalizing them to lie in $[-1,1]$. We then let our network compute the resulting image $\hat{x}$.
    \item We calculate the corresponding structure tensor of $\hat{x}$,
    % \mbox{${\cal S}_s=\begin{bmatrix}(\frac{\partial s}{\partial x})^2 & \frac{\partial s}{\partial x}\frac{\partial s}{\partial y} \\ \frac{\partial s}{\partial x}\frac{\partial s}{\partial y} & (\frac{\partial s}{\partial y})^2 \end{bmatrix}$}
    ${\cal S}_s$.
    % \item We average the four items of ${\cal S}_s$ over the entire image, yielding $\overline{{\cal S}_s}$
    \item The plausible magnitudes range of spatial derivatives varies according to the local nature of the image, e.g., textured regions correspond to larger magnitudes than those corresponding to smooth regions. It therefore makes sense to control a relative magnitude rather than an absolute one, hence we normalize ${{\cal S}_s}$ by
    % $\begin{vmatrix}\frac{\partial h}{\partial x}\frac{\partial h}{\partial y}\end{vmatrix}$,
    $\Sigma_n |h_x[n] h_y[n]|$,
    calculated 
    % and averaged 
    over the corresponding ground truth HR image $x$.
    \item Finally, we calculate the per-image loss as the difference between ${{\cal S}_s}$ and ${\cal S}_\text{d}$, after adjusting the values range of the latter to lie in $[P_5,P_{95}]$, where $P_i$ is the $i^\text{th}$ percentile of ${{\cal S}_s}$ (collected over 10K images): \mbox{${\cal L}_{\text{Struct}}=|{{{\cal S}_s}_{1,1}}-\widehat{{{\cal S}_\text{d}}_{1,1}}|+|{{{\cal S}_s}_{1,2}}-\widehat{{{\cal S}_\text{d}}_{1,2}}|+|{{{\cal S}_s}_{2,2}}-\widehat{{{\cal S}_\text{d}}_{2,2}}|$}, where $\widehat{{{\cal S}_\text{d}}_{i,j}}\triangleq (P_{95}({{{\cal S}_s}_{i,j}})-P_{5}({{{\cal S}_s}_{i,j}})){{\cal S}_\text{d}}_{i,j}/2+\frac{P_{95}({{{\cal S}_s}_{i,j}})+P_{5}({{{\cal S}_s}_{i,j}})}{2}$
\end{enumerate}

